Prompt-based Personalized Federated Learning for Medical Visual Question Answering

We present a novel prompt-based personalized federated learning (pFL) method to address data heterogeneity and privacy concerns in traditional medical visual question answering (VQA) methods. Specifically, we regard medical datasets from different organs as clients and use pFL to train personalized transformer-based VQA models for each client. To address the high computational complexity of client-to-client communication in previous pFL methods, we propose a succinct information sharing system by introducing prompts that are small learnable parameters. In addition, the proposed method introduces a reliability parameter to prevent the negative effects of low performance and irrelevant clients. Finally, extensive evaluations on various heterogeneous medical datasets attest to the effectiveness of our proposed method.

==> temp.tex <==
\begin{table*}[t]
\centering
\begin{minipage}[t]{0.4\linewidth}
    \caption{The results of the Slake.}
    \centering
    \begin{tabular}{cccccc}
    \hline
    \multicolumn{1}{l}{}    & \multicolumn{4}{c}{Subset} & \multicolumn{1}{l}{\multirow{2}{*}{ALL}} \\ 
    \cline{2-5}& Brain& Abdomen& Others & Lung & \multicolumn{1}{l}{}\\ \hline
    VGG+SAN~\cite{liu2021slake}& \multicolumn{4}{c}{-}& 76.1\\ \hline
    VGGseg+SAN~\cite{liu2021slake} & \multicolumn{4}{c}{-}& 75.4\\ \hline
    PubMedCLIP~\cite{eslami2021does}& \multicolumn{4}{c}{-}& 82.5\\ \hline\hline
    AS1& 79.12         & 70.92          & 81.40  & 83.69          & \multirow{5}{*}{-}  \\ \cline{1-5}
    AS2& \textbf{81.32}& 72.34          & 79.07  & 82.98          &      \\ \cline{1-5}
    AS3& 80.22         & \textbf{73.76} & 81.84  & 82.27          &      \\ \cline{1-5}
    AS4& 80.22         & 70.92          & 76.74  & \textbf{84.40} &       \\ \cline{1-5}
    PM & 76.92         & 72.34          & 81.40  & \textbf{84.40} &       \\ \hline
    \end{tabular}
    \label{res-slake}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\linewidth}
    \caption{The results of the VQA-RAD.}
    \centering
    \begin{tabular}{ccccc}
    \hline
    \multicolumn{1}{l}{}   & \multicolumn{3}{c}{Subset}& \multicolumn{1}{l}{\multirow{2}{*}{ALL}} \\ \cline{2-4}
                        & Brain & Abdomen & Chest  & \multicolumn{1}{l}{}                     \\ \hline
    MMBERT~\cite{khare2021mmbert} & \multicolumn{3}{c}{-}  & 77.9                                     \\ \hline
    PubMedCLIP~\cite{eslami2021does} & \multicolumn{3}{c}{-}& 80.0                                     \\ \hline
    CMSA-MTPT~\cite{gong2021cross} & \multicolumn{3}{c}{-}& 80.9                                     \\ \hline
    FITS~\cite{zhang2022type}    & \multicolumn{3}{c}{-}& 82.0                                     \\ \hline\hline
    AS1& \textbf{74.24} & 67.78          & 61.76          & \multirow{5}{*}{-}                       \\ \cline{1-4}
    AS2& 68.18          & 63.33          & 61.76          &                                          \\ \cline{1-4}
    AS3& \textbf{74.24} & 67.78          & 61.76          &                                          \\ \cline{1-4}
    AS4& 69.70          & 67.78          & 60.78          &                                          \\ \cline{1-4}
    PM & \textbf{74.24} & \textbf{68.89} & \textbf{64.71} &                                          \\ \hline
    \end{tabular}
    \label{res-VQARAD}
\end{minipage}
\vspace{-1em}
\end{table*}
